Deep Neural Networks and PIDE discretizations

In this paper, we propose neural networks that tackle the problems of stability and field-of-view of a Convolutional Neural Network (CNN). As an alternative to increasing the network's depth or width to improve performance, we propose integral-based spatially nonlocal operators which are related to global weighted Laplacian, fractional Laplacian and inverse fractional Laplacian operators that arise in several problems in the physical sciences. The forward propagation of such networks is inspired by partial integro-differential equations (PIDEs). We test the effectiveness of the proposed neural architectures on benchmark image classification datasets and semantic segmentation tasks in autonomous driving. Moreover, we investigate the extra computational costs of these dense operators and the stability of forward propagation of the proposed neural networks.

==> images/tstrip.tex <==
\begin{figure}[h!]
\centering
\resizebox{.9\linewidth}{!}{\begin{tikzpicture}[on grid, scale = 0.20]	
  \draw[->, >=angle 90, yslant = -0.5, very thick] (2,-1) -- (-0.5,-1) node[black, pos = -0.25, rotate=-10] {\normalsize $C$};  
  \draw[->, >=angle 90, yslant = -0.5, very thick] (3.1,-1) -- (5.6,-1);
    \draw[->, >=angle 90, yslant = 0.5, very thick] (9,-7) -- (6.5,-7)  node[black, pos = -0.25, rotate=30] {\normalsize $W$};
  \draw[->, >=angle 90, yslant = 0.5, very thick] (10.1,-7) -- (12.6,-7);  
  \draw[->, >=angle 90, yslant = 0.5, very thick] (13,-4) -- (13,-6.5)  node[black, pos = -0.25] {\normalsize $H$};
  \draw[->, >=angle 90, yslant = 0.5, very thick] (13,-2.65) -- (13,-0.5);
  \node[black] at (6,-5.6) {\LARGE $\theta(\mathbf X)$};
  
  \fill[yslant=-0.5,color=cyan] (0,5) rectangle +(6,1);
  \fill[yslant=0.5,color=cyan] (6,-1) rectangle +(1,1);
  \fill[yslant=0.5,xslant = -1, color=cyan](6,6) rectangle +(1,-6); 
  
  %\fill[yslant=0.5,xslant = -1, color=cyan](9,6) rectangle +(1,-6);
  %\fill[yslant=0.5,color=cyan] (9,-1) rectangle +(1,1);   
    
  \draw[yslant=-0.5, opacity = 0.6] (0,0) grid (6,6);
  \draw[yslant=0.5, opacity = 0.6] (6,-6) grid (12,0);
  \draw[yslant=0.5,xslant=-1, opacity = 0.6] (6,0) grid (12,6);

  \draw[yslant=-0.5, black, ultra thick] (0,0) -- (6,0) -- (6,6) -- (0,6) -- cycle;
  \draw[yslant=0.5, black, ultra thick] (6,-6) -- (12,-6) -- (12, 0) -- (6,0);
  \draw[yslant=0.5,xslant=-1, black, ultra thick] (6,6) -- (12,6) -- (12,0);    
  
  \draw[black, very thick, -{Latex[scale=1.2]}](-2,9) to [out=-20,in=110] node[black, pos = -0.3]  {\large $\theta (\mathbf X_i$)}(0.5, 6);
  %\draw[black, very thick, -{Latex[scale=1.2]}](2,10) to [out=-20,in=110] node[black, pos = -0.35]  {\large $\theta (\mathbf X_j$)}(3.7, 7.5);
  
  \fill[yslant=-0.5, color=red!50!yellow, opacity= 0.2](0,0) rectangle +(6,6);
  \fill[yslant=0.5, color=red!50!yellow, opacity= 0.2] (6,-6) rectangle +(6,6);
  \fill[yslant=0.5,xslant=-1, color= red!50!yellow, opacity = 0.2] (12,6) rectangle +(-6,-6);
  
  %\draw[to] (0.5, 6.1) to[bend right=50] node[midway,above] {events};
  %\draw[->, -{Latex[scale=1.5]}] (-2,6) .. controls +(up:7mm) and +(up:7mm) .. (0.5,6.1);
  %\shade[yslant=0.5,right color=yellow,left color=black] (6,-6) rectangle +(6,6);
  %\shade[yslant=0.5,xslant=-1,bottom color=blue, top color=green] (10,5) rectangle +(-5,-5);
  
\end{tikzpicture}
\qquad
\begin{tikzpicture}[on grid, scale = 0.20]	
  \draw[->, >=angle 90, yslant = -0.5, very thick] (2,-1) -- (-0.5,-1) node[black, pos = -0.25, rotate=-10] {\normalsize $C$};  
  \draw[->, >=angle 90, yslant = -0.5, very thick] (3.1,-1) -- (5.6,-1);
    \draw[->, >=angle 90, yslant = 0.5, very thick] (9,-7) -- (6.5,-7)  node[black, pos = -0.25, rotate=30] {\normalsize $W$};
  \draw[->, >=angle 90, yslant = 0.5, very thick] (10.1,-7) -- (12.6,-7);  
  \draw[->, >=angle 90, yslant = 0.5, very thick] (13,-4) -- (13,-6.5)  node[black, pos = -0.25] {\normalsize $H$};
  \draw[->, >=angle 90, yslant = 0.5, very thick] (13,-2.65) -- (13,-0.5);
  \node[black] at (6,-5.6) {\LARGE $\phi(\mathbf X)$};
  
  %\fill[yslant=0.5,xslant = -1, color=cyan](7,6) rectangle +(1,-6);
  %\fill[yslant=0.5,color=cyan] (7,-1) rectangle +(1,1);  
  
  \fill[yslant=0.5,xslant = -1, color=magenta](10,6) rectangle +(1,-6);
  \fill[yslant=0.5,color=magenta] (10,-1) rectangle +(1,1);   
    
  \draw[yslant=-0.5, opacity = 0.6] (0,0) grid (6,6);
  \draw[yslant=0.5, opacity = 0.6] (6,-6) grid (12,0);
  \draw[yslant=0.5,xslant=-1, opacity = 0.6] (6,0) grid (12,6);

  \draw[yslant=-0.5, black, ultra thick] (0,0) -- (6,0) -- (6,6) -- (0,6) -- cycle;
  \draw[yslant=0.5, black, ultra thick] (6,-6) -- (12,-6) -- (12, 0) -- (6,0);
  \draw[yslant=0.5,xslant=-1, black, ultra thick] (6,6) -- (12,6) -- (12,0);  
    
  %\draw[black, very thick, -{Latex[scale=1.2]}](-2,9) to [out=0,in=110] node[black, pos = -0.35]  {\large $\phi (\mathbf X_i$)}(1.5, 6.5);
  \draw[black, very thick, -{Latex[scale=1.2]}](2.5,10) to [out=0,in=110] node[black, pos = -0.35]  {\large $\phi (\mathbf X_j$)}(4.7, 8);
  
  \fill[yslant=-0.5, color=red!50!yellow, opacity= 0.2](0,0) rectangle +(6,6);
  \fill[yslant=0.5, color=red!50!yellow, opacity= 0.2] (6,-6) rectangle +(6,6);
  \fill[yslant=0.5,xslant=-1, color= red!50!yellow, opacity = 0.2] (12,6) rectangle +(-6,-6);
  
  %\draw[to] (0.5, 6.1) to[bend right=50] node[midway,above] {events};
  %\draw[->, -{Latex[scale=1.5]}] (-2,6) .. controls +(up:7mm) and +(up:7mm) .. (0.5,6.1);
  %\shade[yslant=0.5,right color=yellow,left color=black] (6,-6) rectangle +(6,6);
  %\shade[yslant=0.5,xslant=-1,bottom color=blue, top color=green] (10,5) rectangle +(-5,-5);
  
\end{tikzpicture}}

\caption{Pixel strips of embedded versions of $\mathbf X$ with $C$ channels, which are used to compute the kernel entry $\omega(\mathbf X_i, \mathbf X_j)$.} \label{fig:tstrip}
\end{figure}

==> images/tstrip2.tex <==
\begin{figure}[h!]
\centering
\resizebox{.9\linewidth}{!}{\begin{tikzpicture}[on grid, scale = 0.35]	
  \draw[->, >=angle 90, yslant = -0.5, very thick] (2,-1) -- (-0.5,-1) node[black, pos = -0.25, rotate=-10] {\large $C$};  
  \draw[->, >=angle 90, yslant = -0.5, very thick] (3.1,-1) -- (5.6,-1);
    \draw[->, >=angle 90, yslant = 0.5, very thick] (9,-7) -- (6.5,-7)  node[black, pos = -0.25, rotate=30] {\large $W$};
  \draw[->, >=angle 90, yslant = 0.5, very thick] (10.1,-7) -- (12.6,-7);  
  \draw[->, >=angle 90, yslant = 0.5, very thick] (13,-4) -- (13,-6.5)  node[black, pos = -0.25] {\large $H$};
  \draw[->, >=angle 90, yslant = 0.5, very thick] (13,-2.65) -- (13,-0.5);
  \node[black] at (6,-5.6) {\LARGE $\theta(\mathbf X)$};
  
  %\fill[yslant=-0.5,color=cyan] (0,5) rectangle +(6,1);
  %\fill[yslant=0.5,color=cyan] (6,-1) rectangle +(1,1);
  %\fill[yslant=0.5,xslant = -1, color=cyan](6,6) rectangle +(1,-6); 
  
  \fill[yslant=-0.5, color=cyan](0,3) rectangle +(6,1);
  \fill[yslant=0.5,color=cyan] (6,-3) rectangle +(1,1);   
    
  \draw[yslant=-0.5, opacity = 0.6] (0,0) grid (6,6);
  \draw[yslant=0.5, opacity = 0.6] (6,-6) grid (12,0);
  \draw[yslant=0.5,xslant=-1, opacity = 0.6] (6,0) grid (12,6);
  
  \draw[yslant=-0.5, black, ultra thick] (0,0) -- (6,0) -- (6,6) -- (0,6) -- cycle;
  \draw[yslant=0.5, black, ultra thick] (6,-6) -- (12,-6) -- (12, 0) -- (6,0);
  \draw[yslant=0.5,xslant=-1, black, ultra thick] (6,6) -- (12,6) -- (12,0);    
  
  \draw[black, very thick, -{Latex[scale=1.2]}](-1,8.5) to [out=-110,in=140] node[black, pos = -0.1]  {\large $\theta (\mathbf X_i$)}(0, 3.2);
  %\draw[black, very thick, -{Latex[scale=1.2]}](0,8.5) to [out=-10,in=110] node[black, pos = -0.35]  {\large $\theta (\mathbf X_i$)}(1.5, 6.5);
  
   \fill[yslant=-0.5, color=red!50!yellow, opacity= 0.2](0,0) rectangle +(6,6);
  \fill[yslant=0.5, color=red!50!yellow, opacity= 0.2] (6,-6) rectangle +(6,6);
  \fill[yslant=0.5,xslant=-1, color= red!50!yellow, opacity = 0.2] (12,6) rectangle +(-6,-6);
  
  %\draw[to] (0.5, 6.1) to[bend right=50] node[midway,above] {events};
  %\draw[->, -{Latex[scale=1.5]}] (-2,6) .. controls +(up:7mm) and +(up:7mm) .. (0.5,6.1);
  %\shade[yslant=-0.5,right color=gray!10, left color=black!50](0,0) rectangle +(3,3);
  %\shade[yslant=0.5,right color=yellow,left color=black] (6,-6) rectangle +(6,6);
  %\shade[yslant=0.5,xslant=-1,bottom color=blue, top color=green] (10,5) rectangle +(-5,-5);
  
\end{tikzpicture}
\quad \,
\begin{tikzpicture}[on grid, scale = 0.7]	
  \draw[->, >=angle 90, yslant = -0.5, very thick] (1,-0.5) -- (-0.25,-0.5) node[black, pos = -0.25, rotate=-10] {\large $C$};  
  \draw[->, >=angle 90, yslant = -0.5, very thick] (1.6,-0.5) -- (2.8,-0.5);
    \draw[->, >=angle 90, yslant = 0.5, very thick] (4.4,-3.5) -- (3.25,-3.5)  node[black, pos = -0.4, rotate=30] {\large $W'$};
  \draw[->, >=angle 90, yslant = 0.5, very thick] (5.15,-3.5) -- (6.3,-3.5);  
  \draw[->, >=angle 90, yslant = 0.5, very thick] (6.5,-2.1) -- (6.5,-3.25)  node[black, pos = -0.35] {\large $H'$};
  \draw[->, >=angle 90, yslant = 0.5, very thick] (6.5,-1.325) -- (6.5,-0.25);
  \node[black] at (3,-2.8) {\LARGE $\phi(\mathbf{\hat X})$ {\large (subsampled)}};
  
  %\fill[yslant=0.5,xslant = -1, color=cyan](7,6) rectangle +(1,-6);
  %\fill[yslant=0.5,color=cyan] (7,-1) rectangle +(1,1);  
  
  \fill[yslant=0.5,xslant = -1, color=magenta](4,3) rectangle +(1,-3);
  \fill[yslant=0.5,color=magenta] (4,-1) rectangle +(1,1);   
    
  \draw[yslant=-0.5, opacity = 0.6] (0,0) grid (3,3);
  \draw[yslant=0.5, opacity = 0.6] (3,-3) grid (6,0);
  \draw[yslant=0.5,xslant=-1, opacity = 0.6] (3,0) grid (6,3);

  \draw[yslant=-0.5, black, ultra thick] (0,0) -- (3,0) -- (3,3) -- (0,3) -- cycle;
  \draw[yslant=0.5, black, ultra thick] (3,-3) -- (6,-3) -- (6, 0) -- (3,0);
  \draw[yslant=0.5,xslant=-1, black, ultra thick] (3,3) -- (6,3) -- (6,0); 
    
  \draw[yslant=-0.5, opacity = 0.6] (0.5,0) -- (0.5,3);
  \draw[yslant=-0.5, opacity = 0.6] (1.5,0) -- (1.5,3);
  \draw[yslant=-0.5, opacity = 0.6] (2.5,0) -- (2.5,3);
  %\draw[yslant=-0.5] (0,0.5) -- (3,0.5);
  %\draw[yslant=-0.5] (0,1.5) -- (3,1.5);
  %\draw[yslant=-0.5] (0,2.5) -- (3,2.5);
  
  \draw[yslant=0.5,xslant=-1, opacity = 0.6] (3,0.5) -- (6,0.5);
  \draw[yslant=0.5,xslant=-1, opacity = 0.6] (3,1.5) -- (6,1.5);
  \draw[yslant=0.5,xslant=-1, opacity = 0.6] (3,2.5) -- (6,2.5);
	  
  
  \draw[black, very thick, -{Latex[scale=1.2]}](0.6,5) to [out=-20,in=110] node[black, pos = -0.4]  {\large $\phi (\mathbf{\hat X}_j$)}(1.5, 3.7);
  %\draw[black, very thick, -{Latex[scale=1.2]}](2.5,10) to [out=0,in=110] node[black, pos = -0.35]  {\large $\phi (\mathbf X_j$)}(4.7, 8);
	
  \fill[yslant=-0.5, color=red!50!yellow, opacity= 0.2](0,0) rectangle +(3,3);
  \fill[yslant=0.5, color=red!50!yellow, opacity= 0.2] (3,-3) rectangle +(3,3);	  
  \fill[yslant=0.5,xslant=-1, color= red!50!yellow, opacity = 0.2] (6,3) rectangle +(-3,-3);	
  
  
  %\draw[to] (0.5, 6.1) to[bend right=50] node[midway,above] {events};
  %\draw[->, -{Latex[scale=1.5]}] (-2,6) .. controls +(up:7mm) and +(up:7mm) .. (0.5,6.1);
  %\shade[yslant=-0.5,right color=gray!10, left color=black!50](0,0) rectangle +(3,3);
  %\shade[yslant=0.5,right color=yellow,left color=black] (6,-6) rectangle +(6,6);
  %\shade[yslant=0.5,xslant=-1,bottom color=blue, top color=green] (10,5) rectangle +(-5,-5);
  
\end{tikzpicture}}

\caption{Pixel strips of embedded versions of $\mathbf X$ with $C$ channels, which are used to compute the subsampled version of the kernel entry $\omega(\mathbf X_i, \mathbf{\hat X}_j)$.} \label{fig:tstrip2}
\end{figure}
